Comparing Latency and Power Consumption: Quantum vs. Classical Preprocessing

Low latency and low power consumption are the main goals for our future networks. Fiber optics are already widely used for their faster speed. We want to investigate if optical decoding has further advantages to reaching future goals. We have investigated and compared the decoding latency and power consumption of an optical chip and its electronic counterpart built with MOSFETs. We have found that optical processing has a speed and power consumption benefit. For future networks and real-time applications, this can bring huge advantages over our current electronic processors.

==> code.tex <==
import numpy as np
import matplotlib.pyplot as plt
import matplotlib

matplotlib.rcParams['font.size'] = 22

def on_delay(RG, CissVDS, VTH, VGS, Vgp):

    t_don = RG * CissVDS *  np.log((VGS) / (VGS - Vgp))
    return t_don

def off_delay(RG, Ciss, VGS, Vgp):
    term1 = RG * Ciss
    t_doff = term1 * np.log(VGS/Vgp)
    return t_doff

def id(k, vgs, vth, vds):
    id = k * ((vgs-vth)*vds -  (vds**2)/2)
    return id

def id_sat(k, vgs, vth, vds, l):
    vsat = vgs-vth
    id = 0.5 * k * ((vgs-vth)**2) * (1 + l*(vds-vsat))
    return id

def pd(k, vgs, vth, vds):
    pd = 0.5 * k * ((vgs-vth) * (vds ** 2 ) - (1 / 3) * (vds ** 3))
    return pd

RG = 10
CissVDS = 3600 * 10**(-12)
Ciss = 4000* 10**(-12)
VTH = 1.7
Vgp = 2.6

VGS = V_GS = np.linspace(2.6, 15, 100)
t_d_on = []
t_d_off = []
t_d_on = on_delay(RG, CissVDS, VTH, VGS, Vgp)
t_d_off = off_delay(RG, Ciss, VGS, Vgp)

# Plot the turn-on and turn-off delays
plt.figure()
plt.plot(V_GS, t_d_on*1e9, label='Turn-On Delay')
plt.plot(V_GS, t_d_off*1e9, label='Turn-Off Delay')
plt.plot(V_GS, (t_d_on+ t_d_off)*1e9, label='Turn-On + Turn-Off Delay')
plt.xlabel('Gate-Source Voltage (V)')
plt.ylabel('Delay (ns)')
plt.title("Switching Delays for SiRA04DP")
plt.legend()


RG = 20
CissVDS = 1020 * 10**(-12)
Ciss = 1500 * 10**(-12)
VTH = 3
Vgp = 2.1

VGS = V_GS = np.linspace(2.6, 15, 100)
t_d_on = []
t_d_off = []
t_d_on = on_delay(RG, CissVDS, VTH, VGS, Vgp)
t_d_off = off_delay(RG, Ciss, VGS, Vgp)

# Plot the turn-on and turn-off delays
plt.figure()
plt.plot(V_GS, t_d_on*1e9, label='Turn-On Delay')
plt.plot(V_GS, t_d_off*1e9, label='Turn-Off Delay')
plt.plot(V_GS, (t_d_on+ t_d_off)*1e9, label='Turn-On + Turn-Off Delay')
plt.xlabel('Gate-Source Voltage (V)')
plt.ylabel('Delay (ns)')
plt.title("Switching Delays for SiA469DJ")
plt.legend()

pdn = []
pdp=[]
pn = []
pp = []
pnsat = []
ppsat = []
idn = []
idp = []
idnsat = []
idpsat = []
kn = 40
kp = 40
VTHn= 1.7
VTHp = 3
VGS = 5
l = 10*(10**(-3))
VDSn = np.linspace(0, VGS-VTHn, 100)
VDSp = np.linspace(0, VGS-VTHp, 100)
for x in VDSn:
    i = pd(kn, VGS, VTHn, x)
    pdn.append(i)
for x in VDSp:
    i = pd(kp, VGS, VTHp, x)
    pdp.append(i)
for x in VDSn:
    i = id(kn, VGS, VTHn, x)
    idn.append(i)
    p = i * x
    pn.append(p)
for x in VDSp:
    i = id(kp, VGS, VTHp, x)
    idp.append(i)
    p = i * x
    pp.append(p)

VDSnsat = np.linspace( VGS-VTHn, 10, 100)
VDSpsat = np.linspace( VGS-VTHp, 10, 100)
for x in VDSnsat:
    i = id_sat(kn, VGS, VTHn, x, l)
    idnsat.append(i)
    p = i * x
    pnsat.append(p)
for x in VDSpsat:
    i = id_sat(kp, VGS, VTHp, x, l)
    idpsat.append(i)
    p = i * x
    ppsat.append(p)




# Create a figure and axes
#fig, ax1 = plt.subplots()

## Plot power on the left y-axis
#ax1.plot(x, power, 'g-', label='Power')
#ax1.plot(x, pdn, 'r-', label='Power Dissipation')
#ax1.set_xlabel('Drain-Source Voltage (V)')
#ax1.set_ylabel('Power (W)')
#ax1.tick_params('y')

# Create a twin y-axis on the right
#ax2 = ax1.twinx()

# Plot current on the right y-axis
#ax2.plot(x, current, 'b-', label='Current')
#ax2.set_ylabel('Drain-Current (A)')
#ax2.tick_params('y')

# Add legends
#lines, labels = ax1.get_legend_handles_labels()
#lines2, labels2 = ax2.get_legend_handles_labels()
#ax1.legend(lines + lines2, labels + labels2, loc='upper left')
#plt.title("Power and Drain Current of SiRA04DP in Triode Mode")

## Sample data
#x = VDSp
#power = pp
#current = idp

# Create a figure and axes
#fig, ax1 = plt.subplots()

# Plot power on the left y-axis
#ax1.plot(x, power, 'g-', label='Power')
#ax1.plot(x, pdp, 'r-', label='Power Dissipation')
#ax1.set_xlabel('Drain-Source Voltage (V)')
#ax1.set_ylabel('Power (W)')
#ax1.tick_params('y')

# Create a twin y-axis on the right
#ax2 = ax1.twinx()

# Plot current on the right y-axis
#ax2.plot(x, current, 'b-', label='Current')
#ax2.set_ylabel('Drain-Current (A)')
#ax2.tick_params('y')

# Add legends
#lines, labels = ax1.get_legend_handles_labels()
#lines2, labels2 = ax2.get_legend_handles_labels()
#ax1.legend(lines + lines2, labels + labels2, loc='upper left')
#plt.title("Power and Drain Current of SiA469DJ in Triode Mode")









#
#x = VDSp
#xsat=VDSpsat
#power = ppsat
#current = idpsat

# Create a figure and axes
#fig, ax1 = plt.subplots()

# Plot power on the left y-axis
#ax1.plot(x, power, 'g-', label='Power')
#ax1.set_xlabel('Drain-Source Voltage (V)')
#ax1.set_ylabel('Power (W)')
#ax1.tick_params('y')

# Create a twin y-axis on the right
#ax2 = ax1.twinx()

# Plot current on the right y-axis
#ax2.plot(x, current, 'b-', label='Current')
#ax2.set_ylabel('Drain-Current (A)')
#ax2.tick_params('y')

# Add legends
#lines, labels = ax1.get_legend_handles_labels()
#lines2, labels2 = ax2.get_legend_handles_labels()
#ax1.legend(lines + lines2, labels + labels2, loc='upper left')
#plt.title("Power and Drain Current of SiA469DJ in Saturation Mode")
# Display the plot++++++++++++++++++++++++++









pdn1 = []
pdp1=[]
pn1 = []
pp1 = []
pnsat1 = []
ppsat1 = []
idn1 = []
idp1 = []
idnsat1 = []
idpsat1 = []
kn = 25
kp = 250
VTHn= 1.7
VTHp = 3
VGS = 3.3
l = 10*10**(-3)
VDSn = np.linspace(0, VGS-VTHn, 100)
VDSp = np.linspace(0, VGS-VTHp, 100)
for x in VDSn:
    i = pd(kn, VGS, VTHn, x)
    pdn1.append(i)
for x in VDSp:
    i = pd(kp, VGS, VTHp, x)
    pdp1.append(i)
for x in VDSn:
    i = id(kn, VGS, VTHn, x)
    idn1.append(i)
    p = i * x
    pn1.append(p)
for x in VDSp:
    i = id(kp, VGS, VTHp, x)
    idp1.append(i)
    p = i * x
    pp1.append(p)

VDSnsat = np.linspace( VGS-VTHn, 3, 100)
VDSpsat = np.linspace( VGS-VTHp, 3, 100)
for x in VDSnsat:
    i = id_sat(kn, VGS, VTHn, x, l)
    idnsat1.append(i)
    p = i * x
    pnsat1.append(p)
for x in VDSpsat:
    i = id_sat(kp, VGS, VTHp, x, l)
    idpsat1.append(i)
    p = i * x
    ppsat1.append(p)







x1 = np.concatenate([VDSn, VDSnsat])
power1 = pn1+pnsat1
current1 = idn1+idnsat1

# Create a figure and axes
x = np.concatenate([VDSn, VDSnsat])
power = pn+pnsat
current = idn+idnsat

# Create a figure and axes
fig, ax1 = plt.subplots()

# Plot power on the left y-axis
ax1.plot(x, power, 'r-', label='Power at V_GS = 5V', linestyle = "--")
ax1.plot(x1, power1, 'r-', label='Power at V_GS = 3.3V')
ax1.set_xlabel('Drain-Source Voltage (V)')
ax1.set_ylabel('Power (W)')
ax1.tick_params('y')

# Create a twin y-axis on the right
ax2 = ax1.twinx()

# Plot current on the right y-axis
ax2.plot(x, current, 'b-', label='Current at V_GS = 5V', linestyle = "--")
ax2.plot(x1, current1, 'b-', label='Current at V_GS = 3.3V')
ax2.axvline(x=VGS-VTHn, color='gray', linestyle=':')
ax2.axvline(x=3.3-VTHn, color='black', linestyle=':')
x_line = VGS-VTHn
text_x_left = x_line - 0.25
text_y = max(current) - 1
plt.text(text_x_left, text_y, 'Triode')

# Add text on the right side of the vertical line
text_x_right = x_line + 0.1
plt.text(text_x_right, text_y, 'Saturation')

ax2.set_ylabel('Drain-Current (A)')
ax2.tick_params('y')

# Add legends
lines, labels = ax1.get_legend_handles_labels()
lines2, labels2 = ax2.get_legend_handles_labels()
ax1.legend(lines + lines2, labels + labels2, loc='center right')

plt.title("Power and Drain Current of SiRA04DP in Triode and Saturation Mode")


# Plot power on the left y-axis





x1 = np.concatenate([VDSp, VDSpsat])
power1 = pp1+ppsat1
current1 = idp1+idpsat1

# Create a figure and axes
x = np.concatenate([VDSp, VDSpsat])
power = pp+ppsat
current = idp+idpsat

# Create a figure and axes
fig, ax1 = plt.subplots()

# Plot power on the left y-axis
ax1.plot(x, power, 'r-', label='Power at V_GS = 5V', linestyle = "--")
ax1.plot(x1, power1, 'r-', label='Power at V_GS = 3.3V')
ax1.set_xlabel('Drain-Source Voltage (V)')
ax1.set_ylabel('Power (W)')
ax1.tick_params('y')

# Create a twin y-axis on the right
ax2 = ax1.twinx()

# Plot current on the right y-axis
ax2.plot(x, current, 'b-', label='Current at V_GS = 5V', linestyle = "--")
ax2.plot(x1, current1, 'b-', label='Current at V_GS = 3.3V')
ax2.axvline(x=VGS-VTHp, color='gray', linestyle=':')
ax2.axvline(x=3.3-VTHp, color='black', linestyle=':')
x_line = VGS-VTHp
text_x_left = x_line - 0.25
text_y = max(current) - 1
plt.text(text_x_left, text_y, 'Triode')

# Add text on the right side of the vertical line
text_x_right = x_line + 0.1
plt.text(text_x_right, text_y, 'Saturation')
ax2.set_ylabel('Drain-Current (A)')
ax2.tick_params('y')

# Add legends
lines, labels = ax1.get_legend_handles_labels()
lines2, labels2 = ax2.get_legend_handles_labels()
ax1.legend(lines + lines2, labels + labels2, loc='center right')

plt.title("Power and Drain Current of SiA469DJ in Triode and Saturation Mode")











plt.show()

